Binary reachability of timed pushdown automata via quantifier elimination and cyclic order atoms

We study an expressive model of timed pushdown automata extended with modular and fractional clock constraints. We show that the binary reachability relation is effectively expressible in hybrid linear arithmetic with a rational and an integer sort. This subsumes analogous expressibility results previously known for finite and pushdown timed automata with untimed stack. As key technical tools, we use quantifier elimination for a fragment of hybrid linear arithmetic and for cyclic order atoms, and a reduction to register pushdown automata over cyclic order atoms.

==> cfg.tex <==

\section{Construction of the context-free grammar}
\label{sec:cfg}

Let $\P = \tuple {\Sigma, \Gamma, L, X, Z, \Delta}$ be a fractional \TPDA
%with $k$ global clocks $X = \set{x_1, \ldots, x_k}$
%(and thus the same number of stack clocks),
and let its fractional reachability relation be
$$\reach {} {\ell\arr} \ \subseteq \ (\Q \cap [0, 1))^X \times \N^\Sigma \times (\Q \cap [0, 1))^X.$$
%
We construct a context-free grammar $G$ having nonterminals of the form $X_{\ell\arr o}$
for control locations $\ell, \arr$ and an orbit $o$ of $(\Q \cap [0, 1))^{X^2}$
recognising the language
%
\begin{align}
	L(X_{\ell\arr o}) = \setof { w \in \Sigma^* } { \exists (\mu, \nu) \in o \st \mu \reach w {\ell\arr} \nu}.
\end{align}
%
In other words, $X_{\ell\arr o}$ recognises all those (untimed) words which allows $\P$
to go from control state $\ell$, fractional clock values $\mu$, and empty stack,
to control state $\arr$, fractional clock values $\nu$, and empty stack,
for some $\mu, \nu$ in the orbit $o$.
%
(Since $\P$ is fractional,
we do not need the integer value of global clocks in order to describe its runs,
and we can thus safely discard them.)
%
Thus, the untimed language $\languntimed \P {\ell,\arr}$
equals $L(X_{\ell\arr o_0})$, where $o_0 = \set {\mu_0}$ with $\mu_0$ the clock valuation assigning zero to every clock.

\begin{theorem}
	Untimed \TPDA languages are context-free.\lorenzo{justify that the previous transformations preserve the (untimed) language.}
\end{theorem}

\noindent
Assume that there is a clock $x_0$ which is never reset.
For an orbit ${o \subseteq \Q^{X^2}}$
we write $o_1 \subseteq \Q^X$ for its projection onto the first component,
and similarly for $o_2$.
%
\begin{lemma}
	\label{lem:characterisation}
	%Let $\ell, \arr$ be control states of the \trPDA $\P$.
	%
	The relation $\reach {} {\ell\arr}$ is the least relation satisfying the following rules,
	for every fractional valuations $\mu, \nu, \mu', \nu' : (\Q \cap [0, 1))^X$
	and words $w, u, v \in \Sigma^*$:
	%
	\begin{align*}
		&\textrm{\em (input)} &&
			\frac{}{\mu \reach a {\ell\arr} \mu}
				 \qquad &&\textrm{ if } \exists \TPDArule \ell a \arr \in \Delta \\[2ex]
		&\textrm{\em (test)} &&
		\frac{}{\mu \reach \varepsilon {\ell\arr} \mu}
			 \qquad &&\textrm{ if } \exists \TPDArule \ell \varphi \arr \in \Delta \st \mu \models \varphi \\[2ex]
		&\textrm{\em (reset)} &&
		\frac{}{\mu \reach \varepsilon {\ell\arr} \mu [Y \mapsto 0]}
			 \qquad &&\textrm{ if } \exists \TPDArule \ell {\resetop Y} \arr \in \Delta \\[2ex]
		&\textrm{\em (elapse)} &&
			\frac{}{\mu \reach \varepsilon {\ell\arr} \nu}
				 \qquad &&\textrm{ if } \exists \TPDArule \ell \elapse \arr \in \Delta, \delta > 0 \st \nu = \fract {\mu + \delta} \\[2ex]
		&\textrm{\em (push-pop)} &&
			\frac{\mu \reach w {\ell'\arr'} \nu}{\mu \reach w {\ell\arr} \nu}
				  \qquad &&\textrm{ if } \sem {\psi_{\ell\ell'\arr'\arr}^{o_{(\mu, \nu)}}} \neq \emptyset  \\[2ex]
		&\textrm{\em (transitivity)} &&
			\frac{\mu \reach u {\ell\ell'} \mu' \ \mu' \reach v {\ell'\arr} \nu}{\mu \reach {uv} {\ell\arr} \nu}
	\end{align*}
	%
	\begin{align*}
		%\label{eq:pushpop}
		\psi_{\ell\ell'\arr'\arr}^o \ &\equiv\ \!\!\!\!\bigvee_{\delta^\push, \delta^\pop \in \Delta, o' \approx o_1}\!\!\!\!
			\exists \vec x, \vec x', \vec z' \st
				\psi_o(\vec x, \vec x') \wedge \psi_{o'} (\vec z') \wedge \psi_\pop^\Q(\vec x', \vec z') \\[1ex]
		%
		\delta^\push &=
			\TPDArule \ell {\pushopgen \gamma {\fract {z_0} = 0 \wedge \fract {\vec z} = \fract {\vec x} \wedge \floor z = 0}} {\ell'}, \\
		%
		\delta^\pop &=
			\TPDArule {\arr'} {\popopgen \gamma {\psi_\pop^\Q(\vec x, \vec z)}} \arr
	\end{align*}
\end{lemma}
%
In the formula above, variables $\vec x$ describe the fractional values of clocks at the time of push,
$\vec x'$ those at the time of pop,
$\vec z'$ describe the fractional values of stack clocks at the time of pop.
%
Thus, $\psi_o(\vec x, \vec x')$ prescribes that initial-final values are in the orbit $o$,
$\psi_{o'} (\vec z')$ prescribes that the final fractional values of stack clocks are a cyclic permutation $o' \approx o_1$
of the initial clock values $\vec x$ in $o_1$,
and finally $\psi_\pop^\Q(\vec x', \vec z')$ prescribes that final fractional values of global $\vec x'$ and stack clocks $\vec z'$ satisfy the fractional pop constraint.

Based on the characterisation of Lemma~\ref{lem:characterisation},
we can now provide the productions of the grammar.
%
For every nop transition $\TPDArule \ell {a, \varphi, Y, \nop} \arr$
\st $o_1 \models \varphi$ and $o_2 = o_1[Y \mapsto 0]$,
we have a production
%
\begin{align*}
	\textrm{(nop)} & \qquad X_{\ell\arr o} \from a.
%
\intertext{For every time elapse transition $\TPDArule \ell \elapse \arr$, \st $o_1 \approx o_2$ we have a production}
%
	\textrm{(elapse)} & \qquad X_{\ell\arr o} \from \varepsilon.
%
\intertext{
For an orbit $o$ of $\Q^{X^3}$ and $i, j \in \set {1, 2, 3}$,
denote by $o_{ij} \subseteq \Q^{X^2}$ the projection of $o$ to components $i,j$.
%
For every orbit $o$ of $(\Q \cap [0, 1))^{X^3}$, we have a production
}
%
	\textrm{(transitivity)} & \qquad X_{\ell\arr o_{13}} \from X_{\ell\ell'o_{12}} \cdot X_{\ell'\arr o_{23}}.
%
\intertext{Finally, from the push-pop rule we obtain a production}
%
	\textrm{(push-pop)} & \qquad X_{\ell\arr o} \from X_{\ell'\arr'o} \cap I, \textrm{ where }
	I = \setof { w \in \Sigma^*} {\card w_{\tick {x_0}} \in \sem {\psi_{\ell\ell'\arr'\arr}^o}}.
\end{align*}
%
Notice that the language $I$ above is regular, and thus the intersection can be eliminated.

\begin{lemma}[Theorem 4 of \cite{VSS05}] \label{lem:ParIm}
	The Parikh image of the language of a context-free grammar is described by an existential Presburger formula
	computable in linear time.
\end{lemma}

